A Neural ODE Interpretation of Transformer Layers

Transformer layers, which use an alternating pattern of multi-head attention and multi-layer perceptron (MLP) layers, provide an effective tool for a variety of machine learning problems. As the transformer layers use residual connections to avoid the problem of vanishing gradients, they can be viewed as the numerical integration of a differential equation. In this extended abstract, we build upon this connection and propose a modification of the internal architecture of a transformer layer. The proposed model places the multi-head attention sublayer and the MLP sublayer parallel to each other. Our experiments show that this simple modification improves the performance of transformer networks in multiple tasks. Moreover, for the image classification task, we show that using neural ODE solvers with a sophisticated integration scheme further improves performance.

==> backup_scratch.tex <==
\dz{
Main points in this section
\begin{itemize}
    \item baseline original (reimplemented) DEIT TINY (2v50ze6t) acc1: 66.02. Double check if this match the original paper. 
    \item dropout and droppath does not work well with Neural ODE (This is done with \#block=1.)
    \begin{itemize}
        \item (29q2iu34) with droppath, no dropout 27.57
        \item (x76dfx84) no droppath, no dropout 53.33 
        \item (vr7w3hu9) no droppath, with dropout, 40.71
    \end{itemize}
    \item more weight sharing does not mean better performance (The table of different number of stacks)
        \begin{itemize}
            \item 1 block (x76dfx84) time-invariant  53.33
            \item 2 blocks (2lv42jsa)
            \item 3 blocks (57vngj38)
            \item 4 blocks (5vza41xk)
            \item 6 blocks (1mzurm4a)
            \item 12 blocks (2autm2wa) acc1: 70.92
        \end{itemize}
    \item view it as an ODE, we can change to a more sophisticated integrator and improve performance (run time is hurt 4.5h vs. 13.75h)
        \begin{itemize}
            \item 12 blocks (2autm2wa) acc1: 70.92
            \item 12 blocks rk4 (2ho6wyh0) acc1: 72.66 
        \end{itemize}
    \item Ablation study: We can compare the three parallelization implmenetations and focus on one later on in the paper. 
        \begin{itemize}
            \item 12 blocks norm inside dyna (40dvo4bm) acc1: 67.42
            \item 12 blocks two norms (1j1wz519) acc1: 67.03
            \item 12 blocks (2autm2wa) acc1: 70.92
        \end{itemize}
\end{itemize}
}


machine translation

% \dz{
% Main points in this section (All metrics evaluated at step 10260)
% \begin{itemize}
%     \item making the model parallel would reduce validation loss and improve BLEU score with zero dropout. 
%     \begin{itemize}
%         \item (195gg8uj) small sequential transformer  val nll loss: 3.788; bleu 17.0 (17.1@step10k)
%         \item (b0l0p9rj) small (stack 6) transformer with parallelized MLP and attention blocks in both encoder and decoders. val nll loss: 3.626; bleu: 18.2 (17.9@step10k)
%         \item (1n6yfws8) small (stack 6) transformer with parallelized MLP and attention blocks only in encoder. val nll loss: 3.734; bleu score: this evaluation has some problem.  (17.5@step10k)
%     \end{itemize}
%     \item with dropout 0.1, the original transformer performs better
%     \begin{itemize}
%         \item (16xpjci4) small sequential transformer  val nll loss: 3.445; bleu 18.7 (18.7@step10k)
%         \item (163lkwzs) small (stack 6) transformer with parallelized MLP and attention blocks in both encoder and decoders. val nll loss: 3.519; bleu 18.8 (18.5@step10k)
%         \item (ig8qqdis) small (stack 3) transformer with parallelized MLP and attention blocks in both encoder and decoders. val nll loss: 3.695; bleu evaluation has some problem
%         \item (23a85wgc) small (stack 2) transformer with parallelized MLP and attention blocks in both encoder and decoders. val nll loss: 3.822; blue evaluation has some problem. 
%     \end{itemize}
% \end{itemize}
% }


language modelling
\dz{
main points in this section (all results at step 33624)
\begin{itemize}
    \item with dropout, our proposed model does not perform better. 
    \begin{itemize}
        \item (y2mitcym) original small dropout 0.3. val ppl: 101.09
        \item (kky5c7ib) stack6 small dropout 0.3. val ppl: 113.27
        \item (3cii1vh9) original small dropout 0.1. val ppl: 72.72
        \item (39rd2e0g) stack6 small dropout 0.1. val ppl: 76.21
    \end{itemize}
    \item without dropout
    \begin{itemize}
        \item (z8k6q6rd) original small dropout 0.0. val ppl: 65.07
        \item (2qfmt4uw) stack6 small dropout 0.0. val ppl: 60.19
    \end{itemize}
\end{itemize}
}
